Multicomponent Adaptive Sampling Configuration Interaction method in openLOWDIN: positronic and quantum nuclear systems

We present a multicomponent Selective Configuration Interaction (SCI) method based on the deterministic Adaptive Sampling CI (ASCI) algorithm for computing energies and wavefunction properties of molecular systems containing leptons of variable masses, or quantum nuclei. Near-FCI accuracy is achieved by incorporating second-order Epstein-Nesbet perturbation theory or by dressing the Hamiltonian via Davidson's and co-workers shifted-Bk method. We validate the approach through benchmark positronic (e$^+$LiH, e$^+$OH$^-$, e$^+$Mg) and quantum nuclear systems (HCN), establishing a novel protocol for accurate convergence, based on the iterative adaptation of natural orbitals starting from those obtained by considering only cross-particle CISD excitations, to those obtained from SCI variational space, surpassing the accuracy of previous SCI studies. Overall, we show that the present multi-component SCI framework offers a simple, systematically improvable, and cost-effective alternative to traditional CI approaches.

==> supp_mat/buffer_convergence.tex <==
\section{Buffer space size convergence}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.495\linewidth]{supp_mat/Figures/hcn_buffer_sci.pdf}
    \includegraphics[width=0.495\linewidth]{supp_mat/Figures/hcn_buffer_sci+pt2.pdf}
    \includegraphics[width=0.495\linewidth]{supp_mat/Figures/hcn_buffer_scaling.pdf}
    \caption{
    Convergence of SCI energy (\textbf{a}),  SCI+PT2 energy (\textbf{b}), and total elapsed time (\textbf{c}) with respect buffer factor $b_f$, ffor a SCI calculation of HCN with 128k variational configurations. 
    }
    \label{si:fig:buffer_convergence}
\end{figure}

==> supp_mat/core_convergence.tex <==
\section{Core space size convergence}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.495\linewidth]{supp_mat/Figures/hcn_core_convergence.pdf}
    \includegraphics[width=0.495\linewidth]{supp_mat/Figures/hcn_core_scaling.pdf}
    \caption{
    Convergence of SCI energy (\textbf{a}) and amplitude search time scaling (\textbf{b}) with respect to the number of configurations in the core space.
    Horizontal lines were added to show the relative energy changes with respect to the target variational space with half and double the number of configurations. 
    }
    \label{si:fig:core_convergence}
\end{figure}
